Learning Frames from Text with an Unsupervised Latent Variable Model

We develop a probabilistic latent-variable model to discover semantic frames---types of events and their participants---from corpora. We present a Dirichlet-multinomial model in which frames are latent categories that explain the linking of verb-subject-object triples, given document-level sparsity. We analyze what the model learns, and compare it to FrameNet, noting it learns some novel and interesting frames. This document also contains a discussion of inference issues, including concentration parameter learning; and a small-scale error analysis of syntactic parsing accuracy.

==> conclusion.tex <==
\section{Conclusion}

\bocomment{Obvious TODO: write a conclusion}



==> emore/multitable2.tex <==
FN frame & \rotatebox{90}{BrownPTB (100)} & \rotatebox{90}{BrownPTB (400)} & \rotatebox{90}{WSJPTB (100)} & \rotatebox{90}{WSJPTB (400)} & \rotatebox{90}{CrimeNYT (100)} & \rotatebox{90}{CrimeNYT (400)} & \rotatebox{90}{UnifNYT (400)} \\
\hline
Grasp &  & 11 &  & 10 &  &  &  \\
Ingestion &  &  &  &  &  &  & 11 \\
Forming relationships & 16 &  &  &  &  &  & 10 \\
Cause to move in place &  & 15 &  & 10 &  &  &  \\
Encoding &  & 18 &  & 13 &  &  &  \\
Cause to fragment & 10 &  &  &  &  &  &  \\
Differentiation &  & 11 &  & 13 &  &  &  \\
Judgment communication &  &  &  &  &  & 10 &  \\
Attack &  &  &  & 13 &  &  &  \\
Commitment &  &  &  & 12 &  &  &  \\
Cure & 10 &  &  & 11 &  &  &  \\
Cause to amalgamate &  &  &  & 12 &  &  &  \\
Avoiding &  &  &  &  &  & 12 &  \\
Seeking &  &  &  &  &  &  & 15 \\
Education teaching &  & 11 &  & 10 &  &  &  \\
Fluidic motion &  &  &  &  &  &  &  \\
Attempt suasion &  &  &  &  &  & 11 &  \\
Impact &  &  &  &  &  &  &  \\
Name conferral &  &  &  &  &  &  & \textbf{20} \\
Moving in place &  & 14 &  & 10 &  &  &  \\
Sending &  &  &  & 11 &  &  &  \\
Hindering &  &  &  &  &  & 17 &  \\
Grant permission &  &  &  & 11 &  &  &  \\
Judgment &  &  &  &  &  &  & 14 \\
Adorning &  &  &  &  &  &  &  \\
Prevarication &  &  &  &  &  &  &  \\
Scrutiny &  &  &  &  &  &  &  \\
Experiencer focus &  &  &  &  &  & 11 & 10 \\
Arranging &  &  &  & 14 &  &  &  \\
Attaching &  &  &  &  &  &  & 10 \\
Expressing publicly &  &  &  & 12 &  &  &  \\
Light movement & 10 &  &  &  &  &  &  \\
Cogitation &  &  &  &  &  &  &  \\
Residence &  &  &  &  &  &  &  \\
Setting fire & 16 &  &  &  &  &  &  \\
Questioning &  &  &  &  &  &  &  \\
Compatibility &  &  &  &  &  &  &  \\
Theft &  &  &  &  &  &  &  \\
Eclipse &  &  &  &  &  &  &  \\
Coming up with &  &  &  &  &  &  &  \\
Processing materials &  &  &  & 10 &  &  &  \\
Location of light &  &  &  &  &  &  &  \\
Death &  &  &  &  &  &  &  \\
Assessing &  &  &  &  &  &  &  \\
Grooming &  &  &  &  &  &  &  \\
Feigning &  &  &  &  &  &  &  \\
Communication response &  &  &  &  &  &  &  \\
Achieving first &  &  &  &  &  &  &  \\
Desiring &  &  &  &  &  &  &  \\
Inchoative attaching &  &  &  &  &  & 12 &  \\
Mass motion &  &  &  &  &  &  &  \\
Amalgamation &  &  &  &  &  &  &  \\
Cause temperature change &  &  &  & 12 &  &  &  \\
Reading &  &  &  &  &  &  &  \\
Operate vehicle &  &  &  &  &  &  &  \\
Arrest &  &  &  & 12 &  &  &  \\
Quarreling &  &  &  &  &  &  &  \\
Assistance &  &  &  &  &  & 10 &  \\
Duplication &  &  &  &  &  &  &  \\
Beat opponent &  &  &  &  &  &  &  \\


==> experiments.tex <==
\section{Experiments}

\subsection{Dataset}

We have implemented models 1 and 2 and experimented fitting them on the news articles
from the LDC New York Times Annotated Corpus~\citep{nyt_ldc}.
This corpus is useful because news text is relatively easy for current syntactic parsers to analyze,
and the articles have been extensively categorized by hand---every article has a number of descriptor labels.
This makes it easier to extract subsets that are targeted towards specific topics,
making the models' output easier to interpret.
Also, the labels can be used to experiment with Model 3.

Inspired by examples of narrative event structures
in the domain of crime reporting (Chambers and Jurafsky 2009),
and examples in earlier work on scripts (DeJong 1982),
we select news articles for which any of their category labels 
contain any of the words \emph{crime}, \emph{crimes}, or \emph{criminal}.  
This yields 53,182 articles.  
% It turns out the set of topics are a little broader
% than anticipated: these articles have an average of 7.5 category labels each.
We show the most common matching labels, and a sampling of headlines, in Table \ref{cat_counts}.

% We select news articles that have been tagged with the category ``Crimes and Criminals,''
% to see if we can reconstruct some of the narrative typicalities in those stories;
% the domain of crime is often used as an example in the AI literature on scripts.
% It will be interesting to analyze different corpora, but that is not a focus for the current modeling project.

% (Given time, I might try one other type of corpus---perhaps user reviews, or political blog posts.
% Unfortunately, I do not have a corpus of death penalty discussions readily available.
% A thorough treatment of opinion or belief system analysis will have to wait for future work.)
We have been using this dataset, and a smaller development subset of it (2,602 articles) for initial experiments.
Unfortunately, upon further review, there seem to be a number of data quality issues with the metadata---in particular, there are two different system of categories, from different groups within the New York Times,
% (indexing service vs.~an online group), 
and one of them seems to have generally higher quality labels; for example, they disagree whether ``Crime and Criminals'' applies to international terrorism or not, or stories about 9/11 memorials, etc.  When extracting this particualr dataset, we collapsed together all categories,
but for future experiments with the corpus, this and other metadata quality issues may require further consideration.

\begin{table}
  \centering
  \begin{tabular}{|c|l|}
    \hline
    count & category label \\
\hline
48,645 & crime and criminals \\
9,497 & sex crimes \\
6,304 & sentences (criminal) \\
3,892 & war crimes, genocide and crimes against humanity \\
2,818 & organized crime \\
\hline
  \end{tabular}
  \caption{Most common category labels matching query}

%   \begin{tabular}{cc}
% \hline
% 15,737 & terrorism \\
% 14,445 & airlines and airplanes \\
% 14,400 & hijacking \\
% 13,784 & office buildings and commercial properties \\
% 13,759 & world trade center (nyc) \\
% \hline
%   \end{tabular}

  \begin{tabular}{|c|p{5in}|}
\hline
1987-05-05 & JURY SELECTION MAJOR HURDLE IN TRIAL THAT MAY LAST YEARS \\
% 1987-09-05 & PHYSICIAN FROM INDIA IS RAPED AND STABBED TO DEATH IN BROOKLYN \\
1988-02-25 & Moslem Patrol Helps Cut Crime in Brooklyn \\
1991-10-22 & GUILTY PLEAS SET IN U.S. COAL CASE \\
2001-05-30 & 4 GUILTY IN TERROR BOMBINGS OF 2 U.S. EMBASSIES IN AFRICA; JURY TO WEIGH 2 EXECUTIONS \\
2001-10-17 & A Rush for Cipro, and the Global Ripples \\
2003-08-09 & World Briefing | Europe: Northern Ireland: Fund For Bomb Lawsuits \\
2003-10-03 & Bryant's Accuser Won't Have to Testify \\
2004-07-18 & Despite Appeals, Chaos Still Stalks the Sudanese \\
2005-04-01 & World Briefing | Europe: France: Longer Prison Term In Graft Case \\
\hline
\end{tabular}

\caption{Sample of headlines from the dataset.}

\label{cat_counts}
\end{table}


\subsection{Parse preprocessing}

All linguistic analysis is performed as a preprocessing step,
by running the Stanford CoreNLP system,\footnote{\url{http://nlp.stanford.edu/software/corenlp.shtml}}
which performs sentence segmentation, part-of-speech and named entity tagging,
syntactic parsing (Klein and Manning 2003) and conversion to dependencies (de Marneffe et al 2006).
A dependency parse explicitly represents syntactic relations between words, including
the subject and object relationships between a verb and its arguments.
We extract (verb, subject, object) tuples from wherever there is a verb that has
at least one subject or object; if either is missing (e.g.~an intransitive verb, or implied arguments),
the word is assigned a placeholder ``NONE'' symbol.  
We use the Stanford Dependencies' nominative subject and direct object relations for this (\emph{nsubj} and \emph{dobj}).

We selected a random sample of extracted V-S-O tuples to manually assess for accuracy.  A subset are shown in Table \ref{parsing_accuracy}.  We annotated 40 tuples, in context in their respective sentences,
consulting the Stanford Dependency papers (de Marneffe et al 2006, 2008), which have
clear linguistic definitions of the grammatical relations, their conventions for analyzing compound verbs, etc.
Out of 40 tuples, we found 30 had the subject and/or object arguments correct; 6 had one or both wrong; and 4 were incomplete (missing either subject or object)---$75\%$ precision.
We were somewhat surprised to see that most tuples are incomplete.
Complete V-S-O tuples make up only 18.8\% of the tuples, while
43\% are (V,S,\emph{NONE}) and 38\% are (V,\emph{NONE},O).

Finally, we use a vocabulary cutoff to aid efficiency, limiting to the 10,000
most common words across all V-S-O positions.  Words that fall below the
threshold are replaced with an ``OOV'' symbol.
We use the lemmatized (stemmed)
forms of words, as analyzed by the parser.  Unlike standard topic models, we do
not need to remove stopwords, since this is built-in to the grammatical
analysis: the verb-subject and verb-object relations exist directly between
content words.

%Most charitably this is $30/37=81\% (\pm 12\%)$ precision.  Research papers on parsing in NLP regularly claim $\~90\%$ accuracy, but 

% /d/nyt_ldc/preproc/crime % grep -v NONE crime.semtuple | wc -l
%   488331
% /d/nyt_ldc/preproc/crime % wc -l crime.semtuple
%  2591799 crime.semtuple
% /d/nyt_ldc/preproc/crime % echo $((488331*1.0/2591799))
% 0.18841391635693971
% /d/nyt_ldc/preproc/crime % awk '$NF=="NONE"' crime.semtuple|wc -l
%  1120366
% /d/nyt_ldc/preproc/crime % awk '$(NF-1)=="NONE"' crime.semtuple|wc -l
%   983102

\begin{table}
  \centering
  \begin{tabular}{|m{2in}|m{3.5in}|}
    \hline
    correct? & text and V-S-O tuple \\
    \hline
    \textsc{right}: for ``workers,'' only use single head word of the noun phrase
    & In less than an hour , the police and rescue unit ( workers )$_{subj}$ [ found ]$_{verb}$ the ( organ )$_{obj}$ in the tall grass of the field , packed it in ice and took it to the hospital . 
    \\ \hline
    \textsc{right} &
    Mrs. ( Bissell )$_{subj}$ , she said , never [ learned ]$_{verb}$ what her husband did with the money . 
    \\ \hline
    \textsc{incomplete}: ``he'' should be subject of ``defrauded'' since SD uses content verb as head
    & Asked why he had [ defrauded ]$_{verb}$ the insurance ( company )$_{obj}$ and been partners with the mob \ldots
    \\ \hline
    \textsc{wrong}: lists are a known problem case for current parsers
    &
    Guilty on Five Charges Mr. Garcia was found guilty on all five charges against him : ( theft )$_{subj}$ of heroin , possession with intent to [ distribute ]$_{verb}$ heroin , narcotics conspiracy and two ( counts )$_{obj}$ of money laundering . 
    \\
    \hline
  \end{tabular}
  \caption{Example extracted tuples and our annotations in their original sentences (in tokenized form).}
  \label{parsing_accuracy}
\end{table}

We ran CoreNLP on the 53,182 input articles; 
52,254 were processed without error or the software crashing,
yielding 2.6 million V-S-O tuples.

\subsection{Model fitting}

For both Model 1 and 2, we initialize latent variables to random values, then run the Gibbs sampler as described in Section \ref{sec:model}.  Two Gibbs sampling runs are shown for Model 1, on the small and large datasets with $K=100$ frames in both cases.  $\alpha$ is resampled, but $\beta$ is fixed for efficiency reasons.  (It is fixed to $\beta=100$, approximately a value resulting from preliminary experiments when it was resampled.)   We show trace plots for the sampling runs in Figure~\ref{fig:mcmc_fitting}.  It is notoriously difficult to assess MCMC convergence but we attempt some analysis.

Log-likelihood should increase as the Gibbs sampler moves towards a high-density posterior region;
ideally, it should then mix, exploring the posterior.
For the small dataset, it is possible to run 5000 iterations within several hours,\footnote{Implementation in C/Python.}
but unfortunately, it does not seem that log-likelihood has yet leveled off (especially when we view just the last 200 iterations).  (On an even smaller dataset, also shown, it may have leveled off after 5000 iterations.)
On the full dataset, 1000 iterations takes even longer (about 10 hours), and is quite far from convergence.

It should be noted that, even if the log-likelihood levels off, that does not guarantee the MCMC chain is actually mixing---it could be stuck in a local mode.  To properly assess convergence, it is recommended to trace the movement of particular parameters over time.  Unfortunately, in a mixture model the components have identifiability issues, since swapping their labels yields an equivalent likelihood solution; this makes it difficult to interpret movements in individual topic-word or document-topic distributions difficult.

This is disappointing; what is really going on is the Gibbs sampler is acting as an optimizer; if we stop it early, it is simply an incomplete optimizer.  There is a strange phenonenon in the literature that uses Gibbs sampling for topic models: the algorithm is justified on theoretical MCMC grounds of exploring the posterior distribution; but in practice, since the dimensionality is so high, everyone uses it as a stochastic optimizing ``mode-finder'' that then infers a small piece of the posterior distribution around that mode.  Our use of Gibbs sampling largely follows these lines, and suggests that variational or other approaches to inference may be useful.

Final note: as a supplement to log-likelihood, we experimented with tracking the number of changes to $z$ variables
during each iteration---a very simple measure of how much the Gibbs sampler is moving, which we might expect to be higher when it is in a low density region and ``trying'' to get out.  This simple count is computationally attractive because it is substantially faster to compute than the likelihood; we compute it every iteration.  In early iterations, it rapidly decreases as likelihood is rapidly increasing, though by later iterations it is less clear.  Over the iteations where we measure log-likelihood, its correlation with the number of changes is $-0.94$ (and about the same for log(number of changes)).

\begin{figure}[h]
  \begin{center}
    % \includegraphics[width=4in]{images/mcmc_fitting.pdf}
    \includegraphics[width=3.8in,type=pdf,ext=.pdf,read=.pdf]{images/trace.model1.10k.plot}
    \vspace{-.2in}\caption{Tiny dataset (265 documents)}
    \includegraphics[width=3.8in,type=pdf,ext=.pdf,read=.pdf]{images/trace.model1.K=100.a=normal.data=100k.plot}
    \vspace{-.2in}\caption{Small dataset (2600 documents)}
    \includegraphics[width=3.8in,type=pdf,ext=.pdf,read=.pdf]{images/trace.model1.K=100.plot}
    \vspace{-.2in}\caption{Full dataset (52000 documents)}
  \end{center}
  \caption{Model 1 Gibbs sampling runs, on different sized datasets.  The smaller datasets have 5000 iterations, and the large has only 1000.  We show just the last 1000 iterations on the right.  Statistics shown are are (1) number of $z$ changes per iteration, (2) total $p(z,\alpha \mid w, \beta)$ log-posterior (calculated every 10 iterations), and (3) the $\alpha$ parameter, resampled every 50 iterations.
  %   Gibbs sampling log-pseudolikelihood, per iteration.  Before iteration 0 
  % are iterations during the ``token burn-in'' training phase.  
  % Hyperparamter sampling occurs every 50 iterations, starting at iteration 0.}
  }
  \label{fig:mcmc_fitting}
\end{figure}


\subsection{Effects of changing Dirichlet concentration paramters}

TODO explain (1) 99\% mass statistics for Dirichlet sparsity analysis, (2) simulation results, (3) empirical results on changing alpha on Model 1.
Explain (concentration,mean) view of Dirichlets.  
Evidence that we are seeing the asymptotic convergence to Dirichlet process under fixed concentration paramter.  
(Is it Wallach 2009 that mentions this as well; high $K$, low $\alpha$ approximation of DP?)
Explain (derive?) relationship of my ``top-99\% mass'' statistic to asymptotic CRP theory of $O(\alpha\ log N)$ non-empty tables.

With the more complicated models, having several concentration paraemters, it becomes too difficult to tune all 
of them.  This motivated the implementation of posterior sampling of the concentration parameters.

\subsection{Slice sampling Dirichlet concentration parameters}
\label{slice_exper}

This approach is described in section \ref{slice_explain}.
We experimented with several approaches to scheduling the hyperparameter updates, since they are fairly expensive.
In order to best increase overall likelihood over time,
it seemed most useful to a ``token burn-in'' period at the start, leaving the hyperparameters at fixed values then having about 100 iterations of $z$ and $r$ Gibbs sampling iterations; this allows the model to learn reasonable frame distributions, which is the highest dimensional part of the model.  Then we perform hyperparameter resampling every 50 iterations.  It turns out this strategy is similar to the one implemented in the MALLET toolkit.\footnote{\url{http://mallet.cs.umass.edu/}}

For each hyperparameter, we run the slice sampler for 10 iterations, then take the last value of the parameter as a sample from its posterior.  (Johnson 2008 uses 20, and Mallet uses \bocomment{TODO check} by default.)
To choose the number 10, we performed a simulation experiment,
generating 500 artificial Dirichlet-multinomial datasets, and ran a slice sampler on each,
assessing convergence of the distribution across chains to the true distribution.
Figure \ref{fig:qqplots} shows, for each iteration, the distribution of the 500 chains' states against the true posterior, as calculated with a grid approximation on the DCM likelihood.
(This experiment was inspired by Cook et al. (2006)'s simulation testing technique for posterior inference.)
\bocomment{TODO redo and report parameter details.  or better yet, run it on a real z sample}

\begin{figure}[b]
  \begin{center}
  \includegraphics[width=4in]{images/qqplots.pdf}
  \end{center}
  \caption{QQ-plots of the 500 simulated chains, showing their distribution converging to the true posterior over each slice sampling iteration.  Each plot is the QQ-plot of 500 chain states, all at the same iteration.}
  \label{fig:qqplots}
\end{figure}


\begin{figure}[t]
  \begin{center}
    \includegraphics[width=2in]{images/dir_resamp1.pdf}
    \includegraphics[width=4in]{images/dir_resamp2.pdf}
  \end{center}
  \caption{$\alpha$ parameter values over time, when being resampled, from three very different initial positions $\alpha=0.01,\ 1,\ 100$.  The left plot shows the entire history; the right shows from iteration 200 until the end.  
    This is Model 1 on the small dataset. \bocomment{TODO many obvious graph cleanups}}
  \label{fig:dir_resamp}
\end{figure}

The hyperparameter sampling substantially improves likelihood, as noted in previous work.  Interestingly, most of the movement tends to happen early in the MCMC chain, then the hyperparameter stabilizes as the rest of the model is still moving.  We checked if the outcome was initializer dependent by starting three different MCMC chains that were identical except for three different $\alpha$ initializers.  Reassuringly, they all converged on the same region of values.  This robustness to initialization was exactly what we wanted.



\section{Results}

\subsection{Frame lexicons}

\begin{table}[t]\centering
  \begin{tabular}{|p{2in}|p{2in}|p{2in}|}
  \hline
  \input{output_table.tex}
  \end{tabular}
  \caption{\label{output} Example output from Model 1.
  Four of 234 frames are shown; the ten most probable words are shown for each slot type.
  The top ten words take up 30\% to 95\% of the probability mass of the distribution, for these examples.
  }
\end{table}

\begin{table}[t]\centering
  \begin{tabular}{|p{2in}|p{2in}|p{2in}|}
  \hline
  \input{output_table.tex}
  \end{tabular}
  \caption{\label{output} Example output from Model 1.
  Four of 234 frames are shown; the ten most probable words are shown for each slot type.
  The top ten words take up 30\% to 95\% of the probability mass of the distribution, for these examples.
  }
\end{table}


Several frames from Model 1 are shown in Table~\ref{output}.
% The dataset is a corpus of 7,396 New York Times articles annotated with a category called ``Crime and Criminals.''
Several interesting classes of actions are extracted.

\bocomment{TODO: analyze indpendent-tuple versus tuple-in-document.  ($\alpha=\infty$ versus slice-sampled $\alpha$).  Is it more linguistic?  Also, is there a good way to fairly compare topics between models?  greedy 1-1 matching then qualitatively analyze the top-5 pairs?}


\begin{figure}[t]
  \centering
  \includegraphics[width=3in,type=pdf,ext=.pdf,read=.pdf]{images/trace.10_100.plot}
  \label{role_mixing}
  \caption{Model 2 trace plots, $K=10, R=100$, full dataset.}
\end{figure}

Model 2 extracts both role-word distributions, and frames with their frame-argument-role distributions.  
Unlike Model 1, it has two tuning parameters: $K$, the number of frames, and $R$, the number of roles.  Inference is also slower.  After experimenting with various settings, we found that $K=10,R=100$ gave reasonable results: the number of roles was large enough to give interesting word clusters, but unfortunately, the frames are less intelligible.  We would like to have a large number for both $K$ and $R$, but unfortunately, inference is even slower; after 30 hours of runtime $K=10,R=100$ seem to only be starting to mix (Figure \ref{role_mixing}), but $K=100,R=100$ is much worse.  

\begin{figure}[t]
  \centering
  \includegraphics[width=6.5in,type=pdf,ext=.pdf,read=.pdf]{images/rolemat}
  \caption{
  \label{model2}
    Fragment of a Model 2 role-frame matrix; $K=10, R=100$, full dataset.  \emph{(0.787 mass)} indicates that thewords shown comprise 0.787 of the total probability mass of that word multinomial. \bocomment{TODO massive overhaul, this is a quick-and-dirty screenshot from my HTML inspector---bad.  going to all change anyways}}

  \includegraphics[width=7in,type=pdf,ext=.pdf,read=.pdf]{images/rolemodel_frames}
  \caption{Two frames from the above model, with their highest-probability roles for each (V,S,O) argument position---these are two of the frames for which role 61 is active. \bocomment{TODO this is impossible to read\ldots}}

\end{figure}

We show a Model 2 posterior in Figure \ref{model2}.  The role-frame matrix shows the counts that implicitly parameterize the linker $L_{z,a}$ multinomials: the three-dimensional count table $C[frame,\ arg,\ role]$.  One row is a role.  The top words in its multinomial are shown.  Then for each frame, there are counts over the different argument positions it can appear in.  The model naturally segregates verb-only roles from noun roles (since it is relatively rare for the same lemmatized word to be both a noun and a verb).  Furthermore, it learns a sparse set of frame-role linking multinomials---the 0's in this matrix.  The sparsity is controlled by the linker's Dirichlet parameter $gamma$, which is being resampled here.  We show an interesting noun role, that appears in multiple frames, and in different ways---in frame 0 it is usually the subject, but in frames 2 and 3 it is more often the object.

% To further investigate Model 2, given its performance issues, we either have to improve the implementation, or use better inference algorithms, or reduce the dataset.  In the longer term, better inference algorithms that can parallelize are very important---there is some work on parallelized collapsed Gibbs sampling, but its correctness is unclear; variational methods may be more attractive in this regard (and can be faster in themselves), but often have higher memory requirements, can be complicated to derive (though CVB0 (Asuncion et al.~2009) is a promising alternative), and are in general less well-understood than MCMC.  
% (But it is important to find a solution at some point, since scaling to large text datasets is a good way to extract better knowledge from text, as illustrated in web-based information extraction systems like TextRunner or NELL (Banko and Etzioni \ldots Carlson et al. 2010), and large-data uses in NLP in general (language modeling, machine translation, Banko and Brill 2001, etc.)
% 
% Therefore for the short-term, the best route is to investigate a smaller,
% better-targeted corpus.  At the very least, further restrictions or subsets of
% the NYT corpus may yield something of interest.
% There are a number of possible modifications to Model 2 to investigate, and having a
% better dataset will help substantially.

\bocomment{Still want to try PLDA if there's time, but is lower priority than getting the role model to work.}

\subsection{Evaluation}

\bocomment{TODO: try to evaluate against PropBank, MUC, and/or VerbNet/FrameNet.}

\bocomment{Idea: we hypothesize that the lexicons based in linguistic theory (PropBank, VerbNet, FrameNet) differ from information extraction datasets (MUC, ACE, Freitag Acquisitions\ldots) in terms of domain specificity.  We propose this can be tested through the $\alpha$ concentration parameter: if document context doesn't matter and we collpase into a Rooth-like sea-of-tuples model, everything becomes purely syntactic linguistics, so the model should be more like Propbank.  But with stronger document-level constraints, the model becomes more like a topic model, and can learn specifics about the domain.  Maybe.}





==> intro.tex <==
\section{Introduction: Frame induction for corpus analysis}

The use of computational methods to explore research questions in the social
sciences 
has boomed over the past several years, as the volume of
data capturing human communication---e.g.~massive social media data streams---has 
risen to match the ambitious goal of understanding the
behaviors of people and society~\citep{lazer_computational_2009}.
Automated content analysis of text draws
on techniques developed in natural language processing, information retrieval,
and machine learning, and has been applied
to political science, economics, psychology,
and many other areas.
Statistical summaries of language use in a large corpus
can give insight into the opinions, beliefs, and situations communicated in the texts.
In \cite{oconnor_computational_2011}, we overview this field
and note that while state-of-the-art techniques
have great variety in statistical and computational complexity
(as in our own work~\citep{oconnor_tweets_2010,eisenstein_latent_2010,oconnor_mixture_2010,yogatama_predicting_2011,bamman_censorship_2011}, as well as dozens of other examples),
in nearly all cases, researchers restrict their analysis to word and phrase frequencies.
But this falls far short of the insight an expert can achieve when reading a text---in
news, social media,
literature, religious texts,
and other corpora,
the texts
can encode beliefs, opinions, events, arguments, and overarching narrative themes.
Can we automatically extract these from raw text?

As a first step, in this project we focus on \emph{frame and script
learning}---inducing a system of typical events, actors, and actors' roles,
that tend to co-occur within documents.  We use a Bayesian generative modeling
approach, building on previous successes in unsupervised learning of latent
semantic structure in documents and language.

\section{Frames and scripts}

\begin{figure}
\centering
\subfloat[Example from Schank and Abelson (1977)]{
\label{schank}
\includegraphics[width=3in]{images/schank.png}
}
\hspace{.2in}
\subfloat[Example template-filling for Message Understanding Conference (MUC) data; from Chambers and Jurafsky (2011).]{
\label{chambers_muc}
\includegraphics[width=3in]{images/chambers_muc.png}
}
\ \\ 
\subfloat[Two example frames (a.k.a.~templates) learned in Chambers and Jurafsky (2011).  The names of frames and roles were given manually by the researchers, but their noun types, and the typical verbs they are arguments of, are learned automatically from a raw unlabeled corpus.]{
\label{chambers_results}
\includegraphics[width=3.2in]{images/chambers_results.png}
}
\end{figure}

Classic work in artificial intelligence and linguistics
proposes that knowledge has a structured representation of
\emph{frames}, \emph{schemata}, or \emph{scripts} 
(Minsky 1974, Fillmore 1982, Rumelhart 1980, Schank and Abelson 1977).
Figure \ref{schank} shows an example from Schank and Abelson,
where an utterance evokes two levels of analysis: a deep ``knowledge structure'' or ``script,''
that describes the typical aspects of visiting a restaurant;
and a lower-level ``conceptual dependency'' structure, that describes a series of
individual relations and events.

The area of template-filling information extraction, typified by the Message Understanding Conferences
in the late 80's and early 90's,
can be viewed as one practical realization of this idea.  In MUC data, newswire stories are annotated
with one of several templates describing high-level events and their properties;
for example, one MUC corpus consists of news stories about terrorist activities in Latin America,
with a number of templates for the high-level events such as ``bombing,'' ``kidnapping,'' etc.;
see Figure~\ref{chambers_muc} for an example.  One possible application is structured corpus summarization.

We pursue unsupervised learning to automatically induce frames from text,
and to annotate a given text with the frames that underlie it.
Frame-like structured representations have been proposed to model beliefs, opinions, worldviews,
and many other aspects of knowledge, but we focus on
co-occurring events and actor roles, following on the work of Chambers and Jurafsky (2011),
which developed an unsupervised learning approach to induce MUC-style frames from newspaper articles.\footnote{
Note that in both Chambers and Jurafsky (2011), and the MUC approach in general,
there is no temporal or causal ordering to the fine-grained events in
a single text; this contrasts with the usual notion of a script or narrative.
In this work, we stick to this atemporal, ``co-occurring events and actors'' view of a ``script,'' since it is simpler to model. Therefore we use the term ``frame'' in the rest of the document to avoid confusion (though that term is ambiguous in other previous literature).}

Their results are very interesting (Figure \ref{chambers_results}): they were able to reconstruct
some of the hand-built frames from the MUC dataset, and discovered several other ones as well.
Their approach consists of an ad-hoc cascade of several stages of clustering algorithms and many heuristic steps;
unfortunately, it is difficult to replicate, reason about, and extend.

We develop an alternative approach, within the framework
of Bayesian generative statistical models, to accomplish this task.
By taking this approach, we can access a variety of (fairly) well-understood statistical algorithms
for learning and inference, and have principled methods to extend and modify the model
to incorporate document metadata and other sources of information
of great interest for text analysis.
We begin by describing previously existing models for documents and syntactic tuples,
then describe our approach, which builds on these previous advances.



==> model.tex <==
\section{Mixture models of documents, tuples, and roles}
\label{sec:model}

We present a succession of three models to capture
aspects of unsupervised learning of frames.
Initially, we preprocess a corpus of documents into syntactic (verb, subject, object) tuples
using a syntactic parser,\footnote{
Stanford Parser and Dependencies: \url{http://nlp.stanford.edu/software/} (Klein and Manning 2003, de Marneffe et al 2006)}
yielding a dataset of tuples 
$(d, w^{(v)}, w^{(s)}, w^{(o)})_{i=1..N}$.
Our models are fit to this data.

\begin{figure}[p]
  \begin{center}
    \includegraphics[width=6.5in]{images/mymodels_dag.pdf}
  \end{center}
  \caption{Probabilistic DAG notation for our models and related models.  
    Double-border variables are observed.
    Dirichlet priors $\alpha$, $\beta$ 
    (and for Model 2, $\gamma$) are omitted,
    but all multinomials are shown.
    Compare to factor diagrams in Figure \ref{mymodels_factor}.}
  \label{mymodels_dag}
\end{figure}

Figure \ref{mymodels_dag} illustrates the models in probabilistic DAG notation
(Koller and Friedman 2010, Bishop 2006); 
see also the factor graph diagrams in
Figure \ref{mymodels_factor}.

\subsection{Model 1: Document-Tuple}      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

First, we extend the Rooth independent tuple model to incorporate document context,
by giving tuples within the same document a shared multinomial prior over classes.
This amounts to modifying LDA to replace its word generation process with a V-S-O tuple generation process.

For clarity, we notate the three verb, subject, and object
syntactic argument positions
with integers $1,2,3$, and within a tuple reference them with 
an observed variable $a \in \{1,2,3\}$.
We also now call the latent variables ``frames.''
The generative process is:
\begin{itemize}
\item Fix $K$ frames, and Dirichlet priors $\alpha,\beta$
\item \textbf{Frame lexicon:}
  For each frame $k \in 1..K$, and argument position $a\in\{1,2,3\}$,
    \begin{itemize}\item
    Draw word multinomial $\phi^{(a)}_k \sim Dir(\beta)$
    \end{itemize}
  \item \textbf{Document-tuple data:} For each document $d \in 1..D$,
  \begin{itemize}
  \item Draw frame multinomial $\theta_d \sim Dir(\alpha)$
  \item For each tuple $i$ in the document,
    \begin{itemize}
    \item Draw frame indicator $z_i \sim \theta_d$
    \item Draw word triple: for each argument position $a \in \{1,2,3\}$,
      \begin{itemize}
      \item Draw $w^{(a)}_i \sim \phi^{(a)}_{z_i}$
      \end{itemize}
    \end{itemize}
  \end{itemize}
\end{itemize}


% See Figure \ref{model1_fig}.

The per-document prior has the effect of balancing between tuple coherency and document coherency.  The Gibbs update step is to sample from the conditional distribution
\begin{align}
p(z_i \mid w,z_{-i},d,\alpha,\beta) 
&\propto 
\ \textcolor{PineGreen}{p(z_i|d,\alpha)}\ 
p(w^{(v)}|z_i,\beta) p(w^{(s)}|z_i,\beta) p(w^{(o)}|z_i,\beta)
\end{align}
where, as in LDA,
\[ 
\textcolor{PineGreen}{p(z_i|d,\alpha)} 
= \frac{C[z_i,d] + \alpha}{C[d]+\alpha_0} \]
(though the count is over tuples, not word tokens.)

As $\alpha$ increases, the $p(z_i|d)$ term is encouraged to be more and more uniform, and thus have less of an impact on $q(z_i)$; it collapses into the Rooth tuple independence model for $\alpha\rightarrow\infty$.
For a moderate value of $\alpha$, the model encourages tuples in the same document to share the same class.
We hypothesize this will encourage the classes to be not just about linguistic argument categories (as previous tuple modeling work has attempted to model), but also capture related types of events and actions in the corpus, in the same way that LDA on individual words can capture topical themes.

% (where $C_t$ denotes a count over tuples, while $C_w$ a count over word tokens.)
% \frac{C_w[w^{(v)},z_i+\beta}{C_w[z_i]+\beta_0}
% \frac{C_w[w^{(s)},z_i+\beta}{C_w[z_i]+\beta_0}
% \frac{C_w[w^{(o)},z_i+\beta}{C_w[z_i]+\beta_0}


% \begin{figure}[tp]\centering
% \begin{minipage}[b]{3in}\centering
% \includegraphics[width=2.1in]{images/graphical_diagram.pdf}
% \end{minipage}%
% \begin{minipage}[b]{0.45\linewidth}\centering
% \begin{align*}
% \alpha, \beta &= \text{(fixed priors)} \\
% \phi^{(slot)}_k &\sim \text{Dirichlet}(\beta)
%  \ \ \ \ \ k\in\{1..N_{\text{frames}}\},\ slot \in \{v,s,o\}\\
% \theta_d &\sim \text{Dirichlet}(\alpha)
%  \ \ \ \ \ d \in \{1..N_{\text{docs}}\} \\
% z_i &\sim \text{Discrete}(\theta_d)
%  \ \ \ \ \ i \in \{\text{(tokens in doc)}\}\\
% w^{(slot)}_i & \sim \text{Discrete}(\phi^{(slot)}_{z_i})
%  \ \ \ \ \ slot \in \{v,s,o\}
% \end{align*}
% \end{minipage}
% \caption{\label{model1_fig} Model 1: document-tuple generative model.
% For clarity, priors are omitted from the diagram.}
% \end{figure}

\newcommand{\role}[1]{\textsc{#1}}

\subsection{Model 2: Document-Tuple-Role}               %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In Model 1, every class or ``frame'' has completely independent word distributions for the argument positions.
But ideally, we would like higher level roles that summarize word distributions
but cut across the particular types of events.
For example, in the domain of crime stories, we might want to learn
roles for \role{police}, \role{criminal}, and \role{crime} and know that typical events might include 
[v=\role{arrest}, s=\role{police}, o=\role{criminal}] 
and 
[v=\role{commit}, s=\role{criminal}, o=\role{crime}];
those roles might be typically instantiated by words such as
\emph{police, cops, authorities} for \role{police}, or 
\emph{perpetrator, attacker, thief} for \role{criminal}, etc.

We seek to accomplish this by introducing latent \emph{role} variables.
Every role associates with a word multinomial --- a ``role-filler'' distribution ---
while each frame tends to see certain roles in different argument positions 
(the ``linker'' distribution).
The roles intermediate between frames and words, allowing cross-cutting 
roles across frames.

The generative process for Model 2 is:
\begin{itemize}
\item Fix $R$ roles, $K$ frames, and Dirichlet priors $\alpha,\beta,\gamma$
\item \textbf{Frame lexicon:}
\begin{itemize}
  \item For each role $r\in1..R$, 
    \begin{itemize}\item
    Draw word multinomial $\phi_r \sim Dir(\beta)$
    \end{itemize}
  \item For each frame $k\in 1..K$, and argument position $a \in \{1,2,3\}$,
    \begin{itemize}\item
    Draw the ``linker''  $L_{k,a} \sim Dir(\gamma)$, a multinomial over roles: $L_{k,a} \in Simplex(R)$.
    \end{itemize}
\end{itemize}
\item \textbf{Document-tuple data:}
\begin{itemize}
  \item For each document $d \in 1..D$,
    draw frame multinomial $\theta_d \sim Dir(\alpha)$
  \item For each tuple $i$ for document $d$,
  \begin{itemize}
    \item Draw frame indicator $z_i \sim \theta_d$
    \item Draw word triple: for each argument $a \in \{1,2,3\}$,
    \begin{itemize}
      \item (if $a$ is not present in this tuple, skip)
      \item Draw role $r^{(a)} \in L_{z_i,a}$
      \item Draw word $w^{(a)} \in \phi_{r^{(a)}}$
    \end{itemize}
  \end{itemize}
\end{itemize}
\end{itemize}

\noindent
(We have slightly different handling of NONE values than in Model 1: they are skipped and not modeled at all.  If they are explicitly modeled, they take a very large proportion of the probability mass in the role-word distributions, making the results harder to interpret.)

We use a Gibbs sampler that computes updates separately for frame and role variables:
\begin{align}
p(z_i \mid d,z_{-i},r,a; \alpha,\gamma)
&\propto 
p(z_i\mid d,z_{-i},\alpha) \prod_a p(r^{(a)}\mid z_i,a,\gamma)
\\
&=
\frac{\#T[z_i,d] + \alpha}{\#T[d] + \alpha_0}\ 
\prod_a \frac{\#W[r^{(a)},z_i,a]+\gamma}{\#W[z_i,a]+\gamma_0}
\\
p(r^{(a)}\mid z,w^{(a)},a; \gamma,\beta)
&\propto
p(r^{(a)}\mid z,a,\gamma) p(w^{(a)}\mid r^{(a)}, \beta)
\\
&=
\frac{\#W[r^{(a)},z_i,a]+\gamma}{\#W[z_i,a]+\gamma_0}\ 
\frac{\#W[w^{(a)}, r^{(a)}] + \beta}{\#W[r^{(a)}]+\beta_0}
\end{align}

\noindent
where \#T denotes a count over tuples (excluding tuple $i$),
and \#W denotes a count over word tokens; in the first equation, it excludes counts from the three words at tuple $i$; in the second equation, it excludes the word at position $a$ in tuple $i$.
% Since every tuple has three tokens, $\#W[z_i] = 3(\#T[z_i])$.

The algorithm we use is, for one pass through the data: For each tuple $i$, (1) update $z_i$, then (2) for $a=1..3$, update $r^{(a)}$.

Mixing is substantially slower for Model 2 than Model 1,
probably due to the strong dependency between the frame and word roles at a single tuple.
It may be important in the future to investigate alternative inference procedures
that can make larger moves, such as the split-merge sampler (Jain and Neal 2004).

\bocomment{TODO figure out if/how Model 2 is related to the chinese restaurant franchise view of the HDP}

% \clearpage
\subsection{Model 3: Metadata-Frame associations}

Many corpora of analytic interest have some form of observed \emph{document labels},
such as the document's author, 
year of publication, gender of the author, 
political slant of the publication, etc.
Corpus analysis usually involves associating document labels with text 
(e.g.~topical trends over time, difference of writing styles between genders, etc.)
The framework of Partially Labeled LDA \citep{ramage_partially_2011}
learns to associate latent topics with these observed data through a very simple mechanism
of constraining certain topics to only appear in documents having certain labels.
We can easily extend it to our frame models.

PLDA assumes there are $J$ possible binary labels; any set of them may be on for a particular document,
described by binary vector $y^{(d)} \in \{0,1\}^J$.
Every label is globally fixed to be
associated with a particular subset of topics.  
A document's topics are constrained to only include ones that are allowed by the label-topic associations.

Let $M \in \{0,1\}^{J \times K}$ be a binary matrix describing the
label-topic associations, such that $M_{jk}=1$ means that a document with label
$j$ is allowed to use topic $k$.  For example, say $J=3,K=9$ and
% where $y_1$ is a general ``background'' label,
% $y_2$ indicates whether the author is male, and $y_3$ indicates whether the author is female.  Let the association matrix be
\[ M =
  \left(
  \begin{array}{ccccccccc}
    1 & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 & 0 & 1 & 1 & 0 & 0 \\
    0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 1
  \end{array}
  \right) \]
indicating that $y_1$ associates with the first 5 topics, while $y_2$ and $y_3$ associate with two topics each.
Say that $y_1$ is a ``background'' label always on for all documents,
while $y_2$ and $y_3$ indicate whether the author is male or female, respectively.
Then a male author can draw from topics $\{1..7\}$,
while a female author can draw from topics $\{1..5\} \cup \{8,9\}$.

The only change to document generation is to sample the document-topic multinomial 
$\theta^{(d)} \in \mathbb{R}^K$ from a masked prior vector $\alpha^{(d)} \in \mathbb{R}^K$, 
which is zeroed out where the document labels forbid it.
For document $d$, having an observed binary label vector $y^{(d)}$,
\begin{itemize}
  \item Let $\alpha^{(d)}$ be such that
    $\alpha^{(d)}_k=\alpha$ if $M_{jk}=1$ for any $j$ having $y^{(d)}_j=1$;
    otherwise $\alpha^{(d)}_k=0$.
  \item Draw $\theta^{(d)} \sim Dir(\alpha^{(d)})$
\end{itemize}

If the rows of $M$ are mutually exclusive---i.e.~every label's topic set doesn't overlap with any others---the masking operation is equivalent to a matrix multiply $\alpha^{(d)} = (y^{(d)})\transpose M$.  (This suggests a connection between PLDA and the Dirichlet-multinomial regression topic model (Mimno and McCallum, 2008).)

The collapsed Gibbs sampler is trivially easy to implement for PLDA since conjugacy is preserved; one simply zeroes out the disallowed topics when building the conditional Gibbs sampling distribution for $z_i$.  This makes it easy to add PLDA to either Model 1 or Model 2, to associate frames with document characteristics.

A weakness of PLDA is that the label-topic architecture, represented in $M$, has to be specified in advance.  This can be complicated to tune.  Ramage et al. used a setup of several background topics, and a fixed number of topics each for each label, with each labels' topics exclusive.  An interesting extension for future work is to use a Dirichlet process prior to automatically choose the number of topics each label is associated with (also examined by Ramage et al.).

% \clearpage

\subsection{Posterior inference for hyperparameters}
\label{slice_explain}
For exposition, we have indicated the Dirichlet priors $\alpha, \beta, \gamma$ are fixed.
Specifying them manually is, to a certain extent, useful, since they control the degree of sparsity
observed in the posteriors---for example, a small $\alpha$ will tend to decrease the number of topics
used in a document.  But it is possible to fit them to the data as well, to either maximize likelihood
(Wallach 2009, Asuncion 2009, Minka 2009)
or compute a posterior over them (Johnson 2008, TODO find others);
these authors have found that either of these approaches tends to improve model fits.

During inference, we sample these Dirichlet concentration parameters
through slice sampling (Neal 2003),\footnote{
  Using an adaptation of Iain Murray's implementation: 
  \url{http://homepages.inf.ed.ac.uk/imurray2/teaching/09mlss/slice_sample.m}
} an MCMC method for continuous variables that, 
like Metropolis-Hastings, allows one to sample from a complicated distribution
that can only be evaluated at individual points.  But unlike Metropolis-Hastings, it requires no proposal distribution, and very little width tuning, as it adaptively learns a step size.

We interleave the core $z$ and $r$ Gibbs update iterations with hyperparameter Gibbs update steps, using the unnormalied posteriors.  For Models 1 and 2, the $\alpha$ update is through:
\[ p(\alpha\mid z) = p(\alpha) \prod_d p(z_{\{i:\ d_i=d\}} \mid \alpha) \]
where $p(\alpha)$ is assigned to be a vague prior,
and the document
likelihood term $p(z_{\{i:\ d_i=d\}} \mid \alpha)$ is the ``single-path'' Dirichlet-compound multinomial,
derived in Section \ref{dcm_math}.
Update steps for $\beta$ and $\gamma$ are analogous.
For the prior $p(\alpha)$, many authors use a vague Gamma prior that is relatively flat across all positive reals;
but we found success with the even simpler approach of having no prior and only using the 
likelihood term as the unnormalized posterior;
this corresponds to an improper uniform prior having constant density on $\mathbb{R}$.
See section \ref{slice_exper} for details and discussion.




==> old_stuff.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%

% \section{BLA BLA CHANGE}

% My model replaces LDA's exchangeable word generation process with the generation of 
% syntactic and semantic relations; a ``topic''
% consists of a probability distribution over
% relations, roles, and role-filler words, which are generated through the syntactic dependency
% tree.  This approach bridges document-level topic models
% with recent NLP research in unsupervised semantic learning.
% (e.g.~\citet{titov_bayesian_2011}).
% After developing this base model,
% I will incorporate incorporate authors' social contexts to provide rich
% semantic analyses---in this example,
% I would assemble a corpus of social media posts talking about the death penalty
% for users whose profiles declare a conservative or liberal political preference;
% these labels can guide hierarchical priors
% to induce opposing framing structures---political ``spins.''
% The frames shown as boxes in Figure~\ref{dp_framing} correspond to 
% the LDA notion of a latent ``topic,''
% except they specify probability distributions over alternate ways of stating
% the same thing, or groups of statements that co-occur in a typical argument.
% There are numerous variations possible in the framework of probabilistic graphical models.
% 
% My goal is to join two important trends in computational text analysis.
% The first is giving older artificial intelligence theories of frames and narrative structures
% (e.g.~\citet{minsky_framework_1974})
% %,schank_scripts_1977}) 
% a statistical implementation, and learning them directly from data---a 
% challenging problem
% now possible with the tools of several decades of NLP and machine learning research.
% The second is the availability of massive text communications
% endowed with very rich social context---authors,
% their demographics and interests, temporal and spatial structure, etc.
% These two trends pave the way
% for rich analysis of belief structures and worldviews
% across time, space, and social communities.






==> output_table.tex <==
verbs & subjects & objects
\\
\hline\hline
serve, receive, give, impose, face, appeal, spend, seek, get, reduce &
NONE(0.69), judge, OOV, sentence, defendant, court, prosecutor, man, jury, offender &
sentence, term, year, NONE(0.03), time, penalty, probation, conviction, month, fine
\\
\hline\hline
OOV, rule, agree, argue, have, require, apply, refuse, hold, come &
Court, court, judge, OOV, lawyer, law, case, decision, state, prosecutor &
NONE(0.94), OOV, judge, request, time, case, court, hearing, defendant, decision
\\
\hline\hline
sell, use, buy, possess, distribute, fight, take, deal, get, carry &
NONE(0.85), dealer, police, mother, percent, teen-ager, friend, OOV, people, Barry &
drug, cocaine, crack, OOV, heroin, car, worth, marijuana, gas, food
\\
\hline\hline
make, approve, announce, increase, finance, have, propose, support, expand, raise &
NONE(0.73), city, official, plan, Dinkins, Council, Mayor, Koch, administration, budget &
plan, program, proposal, tax, force, budget, system, OOV, increase, NONE(0.01) 
\\
\hline


==> review_lda.tex <==
\section{Document-word mixture model: LDA}

The well-known model of latent Dirichlet allocation \citep{blei_latent_2003}
fits latent mixtures of words over a corpus of documents.
Documents are represented as a mixture of high-level topics,
while their words are generated by the topic-word distributions.

One possible hierarchical generative story for LDA is:
\begin{itemize}
\item Fix $K$ number of topics, and priors $\alpha$, $\beta$
\item \textbf{Topic lexicon:} 
  For each topic $k=1..K$,
  \begin{itemize}
  \item Draw $\phi_k \sim Dir(\beta)$
  \end{itemize}
\item \textbf{Document-word data:}
  For each document $d=1..D$,
  \begin{itemize}
  \item Draw $\theta_d \sim Dir(\alpha)$
  \item For each word token $i=1..N_d$,
    \begin{itemize}
    \item Draw $z_i \sim \theta_d$
    \item Draw $w_i \sim \phi_{z_i}$
    \end{itemize}
  \end{itemize}
\end{itemize}

\noindent
where \begin{itemize}
\item $V=$ the number of distinct words types under consideration,
$K=$ the fixed number of topics, and $D$ the number of documents in the corpus;
\item $\theta_d$ parameterizes a document's discrete distribution over topics; i.e.~$\theta_d \in Simplex(K)$.
\item $\phi_k$ parameterizes a topic's discrete distribution over words; i.e.~$\phi_k \in Simplex(V)$.
\end{itemize}

\begin{figure}\centering
\includegraphics[width=6in]{images/mymodels_factor.pdf}
\caption{\label{mymodels_factor} Factor diagrams for the described models, along with
their respective the Gibbs update conditional factorizations
for their latent variables.  Latent variables are \textcolor{blue}{\textbf{blue}}; the rest are observed.
A factor graph is formally defined as a bipartite graph between variables and factors;
a factor is visually represented here
as a shape surrounding the variables it implicates.
These diagrams only show the discrete variables in the models;
their Dirichlet-multinomial priors are not shown.
}
\end{figure}

An interesting way to think about LDA is to view
the dataset as a giant list of (DocumentID, WordID) pairs for every token:
$(d_i,w_i)$ 
where $i$
indexes across all tokens in the corpus.\footnote{Asuncion et al.~(2009) and Hoffman (1999) take this view.}
The likelihood of all words 
(conditioning on the assignment of tokens to documents, which is taken as fixed)
is:
\begin{align}
p(w|d) 
&= \prod_i p(w_i | d_i) \\
&= \prod_i \sum_{z_i} p(w_i | z_i)\ p(z_i | d_i)  
% p(w|d;\theta,\phi) &
% = \prod_i \sum_{z_i} \phi_k[w_i]\ \theta_d[z_i] 
\end{align}

An effective approach to inference in LDA is collapsed Gibbs sampling 
(Griffiths and Steyvers 2004, Neal 1992),
which only explores settings of 
the per-token latent variables $z$, ``collapsing out'' the $\theta$ and $\phi$ multinomials
by
exploiting Dirichlet-multinomial conjugacy.  
The collapsed Gibbs sampler holds a setting for all $z$ variables,
and sequentially updates one $z_i$ variable at a time, by resampling according to its probability
conditioning on all other variables:
\begin{align}
p(z_i\mid z_{-i}, w, d; \alpha,\beta) \ \propto\ 
  p(z_i \mid z_{-i} ,d, \alpha)\ p(w_i \mid z_i, w_{-i}, \beta)
\end{align}

where $z_{-i}$ and $w_{-i}$ denote all topic indicators and word tokens at all other positions besides $i$.
This approach also conditions on the Dirichlet document-topic and topic-word priors $\alpha$ and $\beta$
(but not $\theta$ or $\phi$, which are implicitly integrated out).

Due to Dirichlet-multinomial conjugacy, the counts of documents, topics, and words are sufficient statistics
 to represent the two probabilities above as:\footnote{Details in section~\ref{dcm_math}.}
\begin{align}
p(z_i=k\mid z_{-i}, w, d; \alpha,\beta)\ \propto\ 
  \frac{ C[k, d_i] + \alpha }{C[d_i] + \alpha_0}\ 
  \frac{ C[w_i, k] + \beta  }{C[k] + \beta_0}
\end{align}

\noindent
where $C$ represents a count over all token positions except for $i$:
$C[k,d_i]$ denotes the count of how many tokens in the document have topic assignment $k$,
$C[d]$ is how many tokens the document contains,
$C[k]$ is how many tokens are assigned to topic $k$ across the whole corpus, and
$C[w_i, k]$ is how many tokens under topic $k$ are the word $w_i$.
These are just marginal counts of the token-level triples $(d,z,w)$.

[And: $\alpha_0=K\alpha, \beta_0=V\beta$; they are the concentration parameters associated with these
 symmetric Dirichlet priors. 
For implementation, $(C[d_i]+\alpha_0)$ can be omitted since it is invariant in $k$.]

This gives a clear interpretation to the probability of assigning $z_i$ to topic $k$:
the left term favors topics that are already prevalent within the document,
while the right term favors topics for which that word is common.
(The constraints are probabilistic and mediated by Bayes rule.)
They might be called document-topic and topic-lexical coherency constraints,
since they tend to favor a specific (soft) set of topics for one document,
and a specific (soft) set of words for one topic;
and they correspond to the two factors in a factor graph view of the probabilistic model
that we illustrate in Figure~\ref{mymodels_factor}.

The collapsed Gibbs sampling algorithm explores the posterior by taking
multiple iterations through the data,
updating the $z_i$ variables in turn, 
while maintaining the necessary marginal count tables.  
The factors in the Figure~\ref{mymodels_factor} diagram
correspond to the highest-dimension count tables that are necessary to maintain.
We will use this simple inference framework for all our models.





==> review_semtuples.tex <==
\section{Semantic tuple mixture models}

Using LDA to model the bag-of-words in a document can recover impressive topical clusters of words,
but our goal is to retrieve deeper frames involving systems of typical events and relationships between
actors in a text.  The key information is relational, and language encodes predicate-argument relationships
in abundance---at the most basic level, as verbs and their arguments.
Verbs often encode events or actions, while nouns usually encode entities.
When a sentence expresses a tuple of (verb, subject, object),
this often encodes an action (verb) performed by an agent (subject), upon or with the object.
Teasing apart these relationships is complicated, and extracting more general forms of the roles
from text is its own subproblem in natural language processing (semantic role labeling (TODO CITE));
but focusing on verbs, subjects, and objects is sufficient to get started in modeling
script-like frames; indeed, this is the focus of the Chambers and Jurafsky work.

There exists a line of work on modeling verb-argument tuples, usually under the guise
of learning \emph{selectional restrictions}, which means the typical classes of arguments for a verb.
For example, ``The man bit the dog''
is unnatural because the subject and object arguments of the verb
\emph{bite} tend to take different classes of noun arguments than are used
here.  This line of work always focuses on modeling (verb, noun) tuples
individually---often extracted from a large corpus with a syntactic parse,
as a preprocessing step---without considering document context.

Looking just at work that uses generative clustering approaches,
Rooth et al (1999) and Pereira et al (1993)
propose a simple class-based model where (verb, object) pair belongs to a particular class, and each class
has separate verb and object word distributions.
Rooth illustrates the model learns broad classes of verbs; for example, one learned class
has its
most probable verbs as \emph{increase as, fall, pay, reduce, rise}
while the the most probable objects are \emph{number, rate, price, cost, level};
they interpret this class as ``scalar change.''

We can generalize the Rooth model to (verb, subject, object) triples, and add some Dirichlet priors, as follows.
$\phi^{(arg)}_k$ denotes a word multinomial for argument type $arg$ and class $k$;
and there are three argument types (verb, subject, object), treated completely separately.
\begin{itemize}
\item
\textbf{Frame lexicon:}
For each $k=1..K$, sample three word multinomials:
$\phi^{(v)}_k, \phi^{(s)}_k, \phi^{(o)}_k \sim Dir(\beta)$
%, where e.g.~$\phi^{(v)}_k$ denotes the distribution for verbs under class $k$; and
\item
\textbf{Tuple data:}
For each tuple $i=1..N$, 
  \begin{itemize}
  \item Draw its class indicator $z_i$ (from a fixed prior),
  \item Draw the three words from their repsective multinomials:
  $w^{(v)}_i \sim \phi^{(v)}_{z_i};\ w^{(s)}_i \sim \phi^{(s)}_{z_i};\ w^{(o)}_i \sim \phi^{(s)}_{z_i}$
  \end{itemize}
\end{itemize}
A factor diagram is shown in Figure~\ref{mymodels}.
This approach models every tuple independently, with no document or other context;
the only thing shared across tuples are the per-class argument word distributions.
More recent work extends Rooth
to model other syntactic relation pairs (O'Seaghdha 2010)
and web-extracted triple relations (Ritter and Etzioni 2010).
The Bayesian framework makes it easy to explore many variants;
we illustrate several of these proposed models in Figure~\ref{model_menagerie}.

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=5in]{images/model_menagerie.pdf}
  \end{center}
  \caption{Several relational tuple models proposed in previous work.  Double-border variables are observed.
    Multinomials are shown but Dirichlet priors omitted.
  The unified notation necessarily conflates distinctions between the authors;
  for example, Ritter models with web-extracted semantic tuples, not syntactic V-S-O tuples.
  }
  \label{model_menagerie}
\end{figure}

There is still more previous work,
including Grenager and Manning (2006) and Titov and Klementiev (2011) which
use a broadly similar Bayesian mixture modeling approaches
to cluster syntactic relations and classes for verb arguments and other syntactic dependencies,
arguing this recovers deeper semantic categories of verbs and other relationships.
Lang and Lapata (2010) introduce a latent logistic regression model for argument structure.


% \citet{rooth99} presents a hidden class model (derived from \cite{pereira93}, but the Rooth paper is much more straightforward), that is used to model either a set of verb-object pairs $(w_{verb}, w{obj})$, or a set of verb-subject pairs $(w_{verb}, w_{obj})$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Common notation
% 
% Lower case roman letters indicate discrete variables:
% 
% $z$: latent semantic class.  $z\in \{1..K\}$
% 
% $w$: word type.  $w \in \{1..V\}$.
% 
% Greek letters indicate multinomial parameter vectors:
% 
% $\theta$: a discrete (multinomial) distribution over classes.  $\theta \in Simplex(K)$
% 
% $\phi$: a discrete (multinomial) distribution over word types.  $\phi \in Simplex(V)$.
% 
% Double circle indicates observed variable.  Single circle indicates latent.
% 
% We use subscripts on multinomials outside the plate, to make the indexing operation clear.  This is a slight violation of standard probabilistic DAG semantics (e.g.~as defined in Koller and Friedman or Bishop).
% 
% $i=\{1..N\}$ indexes tuples.  $v$,$s$,$o$ are arbitrary identifiers for verb, subject, and object slots of tuples.  They could instead be 1,2,3.
% Rooth
% \begin{align}
% z &\ \sim\  \theta_{prior} \\
% w^{(v)} \mid z,\phi &\ \sim\  \phi^{(v)}_z \\
% w^{(n)} \mid z,\phi &\ \sim\  \phi^{(n)}_z
% \end{align}
% 
% O'Seaghdha 3.3
% \begin{align}
% z \mid rel,\theta &\ \sim\  \theta_{rel} \\
% w^{(v)} \mid z,\phi &\ \sim\  \phi^{(v)}_z \\
% w^{(n)} \mid z,\phi &\ \sim\  \phi^{(n)}_z
% \end{align}
% 
% O'Seghdha 3.4
% \begin{align}
% c \mid rel,\eta &\ \sim\  \eta_{rel} \\
% z \mid c,\theta &\ \sim\  \theta_c \\
% w^{(v)} \mid c,\phi &\ \sim\  \phi^{(v)}_c \\
% w^{(n)} \mid z,\phi &\ \sim\  \phi^{(n)}_z
% \end{align}
% 
% O'Seghdha 3.2
% \begin{align}
% z \mid w^{(v)},\theta &\ \sim\  \theta_{w^{(v)}} \\
% w^{(n)} \mid z,\phi &\ \sim\  \phi^{(n)}_z
% \end{align}
% 
% Ritter JointLDA
% \begin{align}
% p(z,w) &\propto p(z,w^{(s)},w^{(o)} \mid w^{(v)}) \\
% &= p(z\mid w^{(v)}) p(w^{(s)}\mid z) p(w^{(o)} \mid z) \\
% z \mid w^{(v)},\theta &\ \sim\  \theta_{w^{(v)}} \\
% w^{(s)} \mid z,\phi &\ \sim\  \phi^{(s)}_z \\
% w^{(o)} \mid z,\phi &\ \sim\  \phi^{(o)}_z 
% \end{align}



